PerFact: Perception-Derived Fact Prompting for 3D Brain MRI Report Generation

Radiology report generation has matured almost entirely on 2D chest radiographs, where the default route to better reports is a larger backbone or a pre-training one on medical data. We revisit that assumption on 3D multi-sequence brain MRI, a volumetric multi-disease regime, and find that the model is not the lever. Zero-shot medical and radiology vision-language models transfer poorly to brain MRI, with chest radiograph specialists failing most conspicuously, and five backbones fine-tuned identically across three model families and an order of magnitude in scale differ only marginally. What determines the quality of the report is the information injected into the prompt. We delegate perception to upstream 3D segmentation and classification, serialize their outputs into a structured fact sentence, and prompt a LoRA-adapted vision-language model with it; we call this \textbf{PerFact}. In a controlled study that fixes the backbone, data split, target reports, and adaptation while varying only the injected grounding, perception-derived facts outperform retrieved prior reports, retrieval becomes redundant once facts are present, and end-to-end predicted facts remain effective without any ground-truth annotation at inference. The residual gap between predicted and oracle facts is explained by the granularity of the facts rather than by the generator. Closed-ended visual question answering comes at no measurable cost to report quality, though the grounding source has little effect on it. On 3D brain MRI, grounding information, not model choice, is the dominant controllable factor in report quality.

==> sections/70_ethics.tex <==
% Ethical Statement -- OPTIONAL, UNNUMBERED (AAAI: \section*).
% Acknowledgments omitted for anonymous submission (would de-anonymize).
\section*{Ethical Statement}
All data are de-identified, publicly released research datasets, with no re-identification
attempted. The imaging comes from public challenge releases and the reports from
RadGenome-Brain MRI; no clinical record was accessed and no new patient data was collected.
The system drafts radiology text as a decision-support aid, not a diagnostic
device: outputs are not clinically validated and require radiologist review. Because reports
stay fluent when wrong, we ground generation in explicit facts and report clinical entity
precision alongside recall. Those facts are themselves predictions, so a report inherits any
error upstream makes; the gap between predicted and oracle facts in Table~\ref{tab:main} is
the size of that exposure. The corpus is narrow, and drawn from challenge datasets rather
than routine practice, so both the case mix and the reporting conventions may differ from a
deployment setting; use elsewhere needs prospective validation on its own data.

